Efficient and Practical Approximation Algorithms for Advertising in Content Feeds

Content feeds provided by platforms such as X (formerly Twitter) and TikTok are consumed by users on a daily basis. In this paper, we revisit the native advertising problem in content feeds, initiated by Ieong et al. Given a sequence of organic items (e.g., videos or posts) relevant to a user's interests or to an information search, the goal is to place ads within the organic content so as to maximize a reward function (e.g., number of clicks), while accounting for two considerations: (1) an ad can only be inserted after a relevant content item; (2) the users' attention decays after consuming content or ads. These considerations provide a natural model for capturing both the advertisement effectiveness and the user experience. In this paper, we design fast and practical 2-approximation greedy algorithms for the associated optimization problem, improving over the best-known practical algorithm that only achieves an approximation factor of~4. Our algorithms exploit a counter-intuitive observation, namely, while top items are seemingly more important due to the decaying attention of the user, taking good care of the bottom items is key for obtaining improved approximation guarantees. We then provide the first comprehensive empirical evaluation on the problem, showing the strong empirical performance of our~methods.

==> main-pratenddefaultcategory.tex <==


\prAtEndRestateii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}For simplicity, we consider a special case where, for each ad $\ad _i$, the rewards $r_{ij}$ are identical, i.e., $r_{ij} = r_i$, for all associated slots $j \in \slots _i$. We first show that the expected reward is non-monotone. It is easy to see that assigning ads sequentially by the order of the slots increases the expected reward. However, assigning a new ad with a zero reward to an earlier slot decreases the expected reward, as it reduces the probability of subsequent ads of being seen. \par We continue to show that the expected-reward function is non-submodular. For any feasible subset $C \subseteq D \subseteq \E $, the marginal gain $g((i,j) \mid C) = f(C+(i,j)) - f(C)$ of adding an edge $(i, j)$ into a set of edges~$C$ is \begin {align*} g((i, j) \mid C) = \rw _i (1-\q )^{j + \nb (j)} - \q \sum _{(i',j') \in C: j' > j} \rw _{i'} (1-\q )^{j' + \nb (j')}. \end {align*} Compared with $g((i ,j) \mid D)$, the first term is clearly non-increasing, but the second term may increase. For example, we have $g((i ,j) \mid C) < g((i ,j) \mid D)$ by letting $D \setminus C$ be ads with zero rewards placed after slot $j$ \emph {and} before other subsequent items. On the other hand, we also have $g((i ,j) \mid C) \ge g((i ,j) \mid D)$ when slot $j$ is ranked after every occupied slot in $D$.\end{proof}

\prAtEndRestateiii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}The proof is similar to the one by \citet {ieong2014advertising} for finely targeted ads, i.e., $|\slots _i| = 1$, for all ads $\ad _i$. The key is to notice that by processing slots backwards, a decision at slot $j$ cannot affect any slot that has not yet been processed, i.e., slots in positions $j'=1,\dots ,j-1$. That is, the user attention for a slot $j'$ does not depend on ads placed later (in slots $j,\dots ,\nV $); additionally, every ad can be re-used as there is no matching constraint. Thus, solving optimally the sequence of sub-problems on slots $j,\dots ,\nV $ with decreasing $j=\nV ,\dots ,1$, yields an optimal solution to \streamadsr . \par The sub-problem for the final slot (i.e., $j=\nV $) is trivial, and \alggback assigns to it the ad with the highest expected reward, if available. Moving backwards to the next slot $j$, \alggback assigns an ad with the highest reward to the slot $j$ only if it improves the total reward, that clearly results in an optimal assignment for this new sub-problem. The proof immediately follows by the above invariant over the backward processing of the slots.\end{proof}

\prAtEndRestateiv*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}At each iteration, $R_j$ remains unchanged if no re-assignment occurs. Hence, consider when an ad $\ad _i$ is re-assigned from slot $\tilde {j}$ to slot $\tilde {j}'$, and let $\tilde {R}_j$ be the revenue after such a re-assignment. First note that our statement does not regard $R_{\tilde {j}'}$, because the sub-problem \streamads -$\tilde {j}'$ is completed after the re-assignment. Clearly, $\tilde {R}_{j} = R_{j}$ for any $j \ge \tilde {j}$. Now let $j < \tilde {j}$. We prove by induction that $\tilde {R}_{j} \le R_{j}$. Recall that $\tau _{j} = \rw _{e_{j}} - \q R_{j}$, and by design of the \alggbackproxy algorithm it holds $\tau _{j} > 0$. \par First, as a base case, when $j = \tilde {j} - 1$, we have \[ \tilde {R}_{j} = (1-\q ) R_{\tilde {j}} \le (1-\q ) (R_{\tilde {j}} + \tau _{\tilde {j}}) = R_{j}. \] In the inductive step, for $j< \tilde {j} -1 $, we have \begin {align*} \tilde {R}_{j} &= (1-\q ) (\tilde {R}_{j+1} + \indicator [e_{j+1} \in \M - (i,\tilde {j})] \tilde {\tau }_{j+1}) \\ &\le (1-\q ) (R_{j+1} + \indicator [e_{j+1} \in \M ] \tau _{j+1}) = R_{j}, \end {align*} where $\tilde {\tau }_{j} = \rw _{e_{j}} - \q \tilde {R}_{j}$. The inequality follows since $\tilde {R}_{j+1} \le R_{j+1}$ holds regardless of $e_{j+1}$ being in $\M $ or not. This completes the proof.\end{proof}

\prAtEndRestatev*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}The marginal gain $g$ of re-assigning ad $\ad _i$ from slot $\tilde {j}$ to slot $j$ is a sum of two terms. The first term is the loss of removing edge $\tilde {e} = (i,\tilde {j})$, and the second term is the marginal reward of adding the new edge $(i,j)$. By \cref {eq:decomp}, we have that \begin {align*} R_j - \tilde {R}_j &= \sum _{j'=j+1}^{\nV } (1-\q )^{j'-j} \left ( \indicator [e_{j'} \in \M ] \tau _{j'} - \indicator [e_{j'} \in \M - \tilde {e}] \tilde {\tau }_{j'} \right ) \\ &= \tau _{i} (1-\q )^{\tilde {j}-j} + \sum _{j'=j+1}^{\tilde {j}-1} (1-\q )^{j'-j} \left ( \indicator [e_{j'} \in \M ] (\tau _{j'} - \tilde {\tau }_{j'}) \right ) \\ &\le \tau _{i} (1-\q )^{\tilde {j}-j} , \end {align*} where $\tilde {R}_j$ is the reward after the removal, and $\tilde {\tau }_{j} = \rw _{e_{j}} - \q \tilde {R}_{j}$. The last two steps follow from \cref {lemma:R}. The claim follows, \begin {align*} g &= \tilde {R}_j - R_j + \rw _{ij} -\q \tilde {R}_j = (1-\q ) (\tilde {R}_j - R_j) + \rw _{ij} -\q R_j \\ &\ge \rw _{ij} -\q R_j - \tau _{i} (1-\q )^{\tilde {j}-j+1} \ge \rw _{ij} -\q R_j - \tau _{i} (1-\q )^{\tilde {j}-j} \end {align*}\end{proof}

\prAtEndRestatevi*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}We prove the claim by induction on slots $j\in [\nV ]$ following the same backward ordering (i.e., $j=\nV ,\dots , 1,0$) adopted by \cref {alg:greedy-backproxy}. Let $\ALG _j$ be the solution of \cref {alg:greedy-backproxy} before performing the $j$-th iteration (i.e., having only processed the slots in positions $\nV ,\dots , j+1$)\footnote {for $j=\nV $ there are no such processed slots, while if $j=0$ then $\ALG _j$ corresponds to the output of~\cref {alg:greedy-backproxy}.}, and $\OPT _j$ be the optimal solution to \streamads (i.e., \OPT ) ignoring the first $j$ slots. Let their objective values for the sub-problem \streamadsj be $R_j := f_j(\ALG _j)$ and $R_j^* := f_j(\OPT _j)$, respectively. And also let the marginal revenue in $R$ be $g_j = R_{j-1} / (1-\q ) - R_j$ at the $j$-th slot, and similarly in $R^*$, $g^*_j = R^*_{j-1} / (1-\q ) - R_j^*$. We then write $\Gamma _i := \tau _i (1-\q )^{\sigma (i)-j}$, for each ad $a_i$ matched in $\ALG _j$. \par Let $\tilde {j}$ be smallest $j$ such that it holds $R_{\tilde {j}} \ge R_{\tilde {j}}^*$. Note that $\tilde {j}$ exists, as $R_\nV = R_\nV ^* = 0$. If $\tilde {j} = 0$, the statement trivially follows. Otherwise, we assume the following hypothesis: for every $j < \tilde {j}$, we can charge the marginal revenue $g^*_j$ of $\OPT _j$ to both $g_j$ and $\{ \Gamma _i \}$ in $\ALG _j$, while maintaining the invariant that every $\Gamma _i$ (corresponding to ad $\ad _i$) in $\ALG _j$ is used at most once among all iterations. This immediately implies \begin {align*} 2 f_j(\ALG _j) &= \sum _{j' > j} g_{j'} (1-\q )^{j'-j} + \sum _{e=(i,j') \in \ALG _j} \Gamma _{i} \\ &\ge \sum _{j' > j} g^*_{j'} (1-\q )^{j'-j} = f_j(\OPT _j) \end {align*} by the decomposition in \cref {eq:decomp}. \par For $j = \tilde {j}$, since $R_j \ge R_j^*$, it is sufficient to consider only the marginal gains $\{ g_j \}$, as it holds $R_j \ge R_j^*$. Now, for the next smaller $j$ in an inductive step, we have the following cases. \par \textbf {Case 1}. $\OPT _{j-1} = \OPT _{j}$, that is, \OPT does not include any new ad for its $j$-th slot. If our \ALG also does not select any item for the $j$-th slot, then the inductive step clearly holds. \par Otherwise, notice that~\cref {alg:greedy-backproxy} (re-)assigns an ad only if $g_{LB} > 0$ by \cref {lemma:LB}. Hence, the overall revenue (i.e., $R_{j-1}/(1-\q )$) only increases, and therefore our hypothesis holds also for this case. \par \textbf {Case 2}. $\OPT _{j-1} = \OPT _{j} + e^*$, where $e^* = (i^*, j)$, that is the optimal solution assigns ad $i^*$ to the $j$-th slot. \par \textbf {Case 2.1}. If our \ALG (re-)assigns ad $i$ to slot $j$, i.e., matching the edge $e=(i, j)$, then by the greedy criterion (\cref {eq:greedy-proxy}), we have \[ \rw _e - \Gamma _i \ge \rw _{e^*} - \Gamma _{i^*} . \] Therefore, we can use both $\Gamma _{i^*}$ and $g_j$ to charge for $\rw _{e^*}$. That is, \begin {align*} g_j + \Gamma _{i^*} &\ge \rw _e - \Gamma _{i} - q R_j + \Gamma _{i^*} \ge \rw _{e^*} - q R_j^* = g^*_j, \end {align*} where the first inequality follows by \cref {lemma:LB}, and the second follows by the greedy rule and the fact that $R_j < R_j^*$ (as $j < \tilde {j}$). Note that if ad $\ad _{i^*}$ was not matched in $\ALG _j$ then $\Gamma _{i^*} = 0$, or otherwise, we increase the number of charges on $\Gamma _{i^*}$ by one. \par \textbf {Case 2.2}. $\ALG _{j-1} = \ALG _{j}$. The greedy choice and its inequalities from Case 2.1 still apply, but fail to produce a positive lower bound. That is, $g_{LB} = \rw _e - \Gamma _{i} - q R_j \le 0$ for each $e=(i,j)$. Therefore, it is sufficient to only pay $\Gamma _{i^*}$ for this case.~\ilie {Question: is this the same $i^*$ of $e^*$ or is this the $i^*$ on which $g_{LB}$ is evaluated?}\guangyi {The former.}\ilie {Maybe stupid question, can it be that $\Gamma _{i^*}=0$ and for all other iterations, including the one for this case, $g_{LB}<0$?}\guangyi {Do you mean $\Gamma _{i^*}=0$ for all iterations? I think it doesn't matter and we can pay $\Gamma _{i^*}=0$ even if it is zero. In any case we have $\rw _e - \Gamma _{i} - q R_j + \Gamma _{i^*} \ge \rw _{e^*} - q R_j^*$ and we can get $g^*_j$ covered.} \par In Case 2, we use each $\Gamma _i$ at most once because \OPT contains at most one edge incident to ad $\ad _i$, given the matching constraint. Furthermore, $\tau _i$ is non-decreasing after re-assigning either ad $\ad _i$ (by design of \alggbackproxy ), or other ads $\ad _{i'}$ (by \cref {lemma:R}), so the payments in prior iterations remain valid, completing the proof.\end{proof}

\prAtEndRestatevii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}Fix $\q =0$, and then \streamads is reduced to a maximum weighted matching problem (\mwm ). It is well known that a greedy algorithm cannot do better than 2-approximation for \mwm . Concretely, let $\nV =2$. Create two ads $\ad _1, \ad _2$ with slots $\slots _1 = \{1,2\}$ and $\slots _2 = \{2\}$, respectively. Set rewards $\rw _{11} = \rw _{22} = 1$ and $\rw _{12} = 1+\epsilon $. Thus, a backwards-greedy algorithm yields a revenue of $1+\epsilon $ by assigning $\ad _1$ to the 2-nd slot, while the optimum assignment yields 2. The ratio approaches 2 for an arbitrary small $\epsilon $.\end{proof}

\prAtEndRestateviii*

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}The proof is similar to \cref {thm:greedy-streamads}, except that we need a different inequality for the Case 2 therein. Though \cref {alg:greedy-back} does not use the values $\tau _i$, we use such values here only for the analysis, and assume that \cref {alg:greedy-back} updates the values $\tau _i$ as from \cref {thm:greedy-streamads}. Recall that $\Gamma _i := \tau _i (1-\q )^{\sigma (i)-j}$. \par Suppose that at slot $j$, $\OPT _{j-1} = \OPT _{j} + e^*$, where $e^* = (i^*, j)$. If our \ALG (re-)assigns edge $e=(i, j)$, then by the greedy criterion, \begin {align*} g_{i} &\ge g_{i^*} \\ \rw _{ij} -\q R_j - \kappa _{ij} &\ge \rw _{i^*j} -\q R_j - \kappa _{i^*j}, \end {align*} where $g_i$ denotes the marginal reward of (re-)assigning ad $\ad _i$, and $\kappa _{ij} := \rw _{ij} -\q R_j - g_{i}$. By \cref {lemma:LB}, we have for any $i$, \[ g_i \ge \rw _{ij} -\q R_j - \Gamma _i \quad \implies \quad \Gamma _i \ge \kappa _{ij}. \] Therefore, we can use both $\Gamma _{i^*}$ and $g_j$ to charge for $\rw _{i^*j}$. That is, \begin {align*} g_j + \Gamma _{i^*} &= \rw _{ij} -\q R_j - \kappa _{ij} + \Gamma _{i^*} \\ &\ge \rw _{i^*j} -\q R_j - \kappa _{i^*j} + \Gamma _{i^*} \\ &\ge \rw _{i^*j} -\q R_j^* - \kappa _{i^*j} + \Gamma _{i^*} \\ &\ge \rw _{i^*j} -\q R_j^* = g^*_j, \end {align*} where the inequalities follow by the greedy rule, the fact that $R_j < R_j^*$, and \cref {lemma:LB}, respectively. \par The claim follows by charging every $g^*_j$ to $g_j$ and $\{ \Gamma _i \}$, and noting that every $\Gamma _i$ is used at most once among all iterations. We omit the details for the other cases, as they follow from \cref {thm:greedy-streamads}.\end{proof}

